TaRL: Learning General and Physical Rewards from Tactile Demonstrations

Contact-rich manipulation requires robots to sequence precise contacts, maintain stable grasps, and apply directed forces. Reinforcement learning (RL) can acquire such behaviors automatically, but its performance hinges on reward design: sparse rewards reduce the learning efficiency, while dense rewards are hard to specify. Visual reward learning addresses this by inferring rewards from action-free demonstrations. Because it conditions only on visual observations, it fails to capture rewards beyond visual goals. We propose Tactile Reward Learning (TaRL), a framework that learns rewards from tactile demonstrations. TaRL takes a sequence of tactile deformation maps as input, and regresses task-completion progress from both successful and failed demonstrations. Because TaRL captures local robot-object interaction, it provides informative feedback to learn firm grasps and correctly directed forces; meanwhile, it is robust to changes in scene layout such as object position. We evaluate TaRL on four manipulation tasks in simulation and two in the real world. Used as a shaping reward, it substantially improves both sample efficiency and final success rate, raising success on Nut threading from 34% to 56% in simulation and on cube pickup from 37% to 97% in the real world. Combining tactile with visual rewards improves performance further. TaRL also generalizes across object instances: trained on box placement and directly deployed to can placement, it significantly improves policy learning on the new task. Project page is available at https://embodiedai-ntu.github.io/tarl.

==> src/fig_rl_baseline.tex <==
\begin{figure}[h]
    \centering
    \begin{adjustbox}{width=\linewidth}
    \tb{@{}cccc@{}}{0.1}{
    \imw{figures/main_experiment_peg}{0.25} & \imw{figures/main_experiment_peg}{0.25} &
    \imw{figures/main_experiment_nut}{0.25} & \imw{figures/main_experiment_gear}{0.25} \\ [-2pt]
    (a) Pick and Place & (b) Peg Insertion &
    (c) Gear Assembly & (d) Nut-Thread Insertion
    }
    \end{adjustbox}
    \caption{
     a
    }
    \label{fig:rl_baseline}
\end{figure}

==> src/fig_sim_to_real.tex <==
\begin{wrapfigure}{r}{0.45\textwidth}
  \vspace{-2.5em}
  \centering
  \begin{adjustbox}{width=\linewidth}
    \tb{@{}cc@{}}{0.05}{
      \imw{figures/sim_to_real_box}{0.5} & 
      \imw{figures/sim_to_real_nut}{0.5} \\[-2pt]
      {\footnotesize (a) Stable Grasp} & 
      {\footnotesize (b) Rotation} \\
    }
  \end{adjustbox}
  \caption{
    a
  }
  \label{fig:sim_to_real}
  \vspace{-4em}
\end{wrapfigure}

==> src/fig_tacreward_evaluate.tex <==
\begin{figure}[h]
    \centering
    \begin{adjustbox}{width=\linewidth}
    \tb{@{}cccc@{}}{0.1}{
    \imw{figures/box_rolling}{0.25} & \imw{figures/peg_rolling}{0.25} &
    \imw{figures/gear_rolling}{0.25} & \imw{figures/nut_rolling}{0.25} \\ [-2pt]
    (a) Pick and Place & (b) Peg Insertion &
    (c) Gear Assembly & (d) Nut-Thread Insertion
    }
    \end{adjustbox}
    \caption{
     a
    }
    \label{fig:tacreward_evaluation}
\end{figure}

==> src/fig_task_generalization.tex <==
\begin{figure}[t]
  \centering
  \setlength{\tabcolsep}{2pt}
  \renewcommand{\arraystretch}{0.5}
  \newcommand{\rowlabel}[1]{\adjustbox{valign=c}{\rotatebox{90}{\small\textbf{#1}}}}
  \begin{tabular}{cccc}
    \rowlabel{Box Placement} &
      \includegraphics[width=0.30\linewidth, valign=c]{figures/task_generalization/cross_box_to_gear.png} &
      \includegraphics[width=0.30\linewidth, valign=c]{figures/task_generalization/cross_box_to_nut.png} &
      \includegraphics[width=0.30\linewidth, valign=c]{figures/task_generalization/cross_box_to_peg.png} \\[2pt]
    & {\small \textbf{$\rightarrow$ Gear Assembly}} & {\small \textbf{$\rightarrow$ Nut Threading}} & {\small \textbf{$\rightarrow$ Peg Insertion}} \\
    \rowlabel{Gear Assembly} &
      \includegraphics[width=0.30\linewidth, valign=c]{figures/task_generalization/cross_gear_to_box.png} &
      \includegraphics[width=0.30\linewidth, valign=c]{figures/task_generalization/cross_gear_to_nut.png} &
      \includegraphics[width=0.30\linewidth, valign=c]{figures/task_generalization/cross_gear_to_peg.png} \\[2pt]
    & {\small \textbf{$\rightarrow$ Box Placement}} & {\small \textbf{$\rightarrow$ Nut Threading}} & {\small \textbf{$\rightarrow$ Peg Insertion}} \\
    \rowlabel{Nut Threading} &
      \includegraphics[width=0.30\linewidth, valign=c]{figures/task_generalization/cross_nut_to_box.png} &
      \includegraphics[width=0.30\linewidth, valign=c]{figures/task_generalization/cross_nut_to_gear.png} &
      \includegraphics[width=0.30\linewidth, valign=c]{figures/task_generalization/cross_nut_to_peg.png} \\[2pt]
    & {\small \textbf{$\rightarrow$ Box Placement}} & {\small \textbf{$\rightarrow$ Gear Assembly}} & {\small \textbf{$\rightarrow$ Peg Insertion}} \\
    \rowlabel{Peg Insertion} &
      \includegraphics[width=0.30\linewidth, valign=c]{figures/task_generalization/cross_peg_to_box.png} &
      \includegraphics[width=0.30\linewidth, valign=c]{figures/task_generalization/cross_peg_to_gear.png} &
      \includegraphics[width=0.30\linewidth, valign=c]{figures/task_generalization/cross_peg_to_nut.png} \\[2pt]
    & {\small \textbf{$\rightarrow$ Box Placement}} & {\small \textbf{$\rightarrow$ Gear Assembly}} & {\small \textbf{$\rightarrow$ Nut Threading}} \\
  \end{tabular}
  \caption{\textbf{Cross-task generalization of tactile reward models.} Each row
    corresponds to a source model (box / gear / nut / peg) deployed
    zero-shot on the three other target tasks. Trajectory with similar tactile pattern shows generalization, which can directly distinguish successful and failure trajectories on different tasks.}
  \label{fig:cross_task_grid}
\end{figure}

==> src/fig_task_generalization_and_sim2real.tex <==
\begin{figure}[h]
  \centering
  \begin{adjustbox}{width=\linewidth}
  \tb{@{}c@{}}{0.05}{
      \imw{figures/generalization_and_sim2real}{0.9} \\
  }
  \end{adjustbox}
  \caption{
    \textbf{Tactile rewards transfer beyond training conditions.} \textbf{Left:} \method{} generalizes to novel object instances in pick-and-place, improving the online RL training efficiency. \textbf{Right:} \method{} trained in simulation transfers directly to the real world.
  }
  \label{fig:task_generalization}
  % \centering
  % \begin{minipage}[b]{0.25\textwidth}
  %     %\vspace{-1.2em}
  %     \centering
  %     \begin{adjustbox}{width=\linewidth}
  %     \tb{@{}c@{}}{0.05}{
  %         \imw{figures/task_generalization_bowl}{1.0} \\
  %         bowl \\
  %     }
  %     \end{adjustbox}
  %     \caption{
  %       \method{} generalizes across different tasks.
  %     }
  %     \label{fig:task_generalization}
  %     %\vspace{-1em}
  % \end{minipage}
  % \hfill % Adds horizontal space between the minipages
  % \begin{minipage}[b]{0.74\textwidth}
  %   \centering
  %   \begin{adjustbox}{width=\linewidth}
  %     \tb{@{}c@{}}{0.05}{
  %       \imw{figures/sim_to_real}{1.0} \\
  %     }
  %   \end{adjustbox}
  %   \caption{
  %     a
  %   }
  %   \label{fig:sim_to_real}
  % \end{minipage}
\end{figure}


==> src/fig_tsne_tactile.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=0.55\linewidth]{figures/tsne_success_trajectories.png}
  \caption{t-SNE projection of per-trajectory tactile descriptors for
    successful rollouts of the four tasks. Each point is one trajectory
    summarized by per-taxel max-force and contact-persistence statistics
    pooled over time; PCA to $50$ dimensions precedes t-SNE
    (perplexity $30$). Clusters separate cleanly by task, with the largest
    residual overlap between gear and nut pick-place.}
  \label{fig:tactile_tsne}
\end{figure}


==> src/fig_visual_tactile_comparison.tex <==
\begin{figure}[t]
  % \vspace{-2em}
  \centering
  \begin{adjustbox}{width=\linewidth}
    \tb{@{}cc@{}}{0.05}{
      \imw{figures/visual_rewind_peg}{0.55} & 
      \imw{figures/rgb_tactile_rl}{0.45} \\
      {\footnotesize (a) Predicted rewards} & 
      {\footnotesize (b) Online RL performance} \\
    }
  \end{adjustbox}
  \caption{
    \textbf{Comparison of visual and tactile reward.}
  }
  \label{fig:visual_tactile}
\end{figure}

==> src/fig_visual_tactile_viz.tex <==
\begin{figure}[h]
    \centering
    \begin{subfigure}{0.99\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/visual_tactile_comaprison}
        \caption*{Peg Insertion}
    \end{subfigure}\\[4pt]
    \begin{subfigure}{0.99\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/gear_visual_tactile_viz}
        \caption*{Gear Assembly}
    \end{subfigure}\\[4pt]
    \begin{subfigure}{0.99\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/nut_visual_tactile_viz}
        \caption*{Nut Threading}
    \end{subfigure}\\[4pt]
    \begin{subfigure}{0.99\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/block_visual_tactile_viz}
        \caption*{Box Placement}
    \end{subfigure}
    \caption{
    \textbf{Tactile rewards generalize to unseen object positions.} Predicted reward (y-axis) along a successful rollout
    for the tactile (blue) and visual (orange) reward models, shown for
    each of the four tasks (top to bottom: Peg Insertion, Gear Assembly,
    Nut Threading, and Box Placement). Each panel reports rewards at the
    training object position and at object positions not seen during
    training. At the training position, both models produce informative,
    monotonically increasing rewards. At novel positions, the tactile
    reward preserves this structure across all four tasks, whereas the
    visual reward collapses and no longer tracks task progress.
    }
    \label{fig:visual_tactile_viz}
\end{figure}

==> src/tab_training_hyperparameter.tex <==
\begin{table}[H]
\centering
\begin{tabular}{l c c c}
\toprule
\multicolumn{4}{l}{\textbf{Hyperparameter}} \\
\midrule

\multicolumn{4}{l}{\textbf{PPO}} \\
\midrule
Algorithm                          & \multicolumn{3}{c}{A2C-continuous (PPO)} \\
Mini-epochs per update             & \multicolumn{3}{c}{4} \\
Clip ratio ($\epsilon$)            & \multicolumn{3}{c}{0.2} \\
Discount factor ($\gamma$)         & \multicolumn{3}{c}{0.995} \\
GAE parameter ($\lambda$)          & \multicolumn{3}{c}{0.95} \\
Entropy coefficient                & \multicolumn{3}{c}{0.005} \\
Critic coefficient                 & \multicolumn{3}{c}{2.0} \\
Bounds loss coefficient            & \multicolumn{3}{c}{0.0001} \\
Value bootstrap                    & \multicolumn{3}{c}{True} \\
Clip value                         & \multicolumn{3}{c}{True} \\
Normalize advantage / input / value & \multicolumn{3}{c}{True} \\
Gradient norm clipping             & \multicolumn{3}{c}{1.0} \\
Minibatch size                     & \multicolumn{3}{c}{512} \\
Horizon length                     & \multicolumn{3}{c}{128} \\

\midrule
\multicolumn{4}{l}{\textbf{Network (Actor--Critic, asymmetric)}} \\
\midrule
MLP hidden units                   & \multicolumn{3}{c}{[512, 128, 64]} \\
MLP activation                     & \multicolumn{3}{c}{ELU} \\
Recurrent core                     & \multicolumn{3}{c}{LSTM (1024 units, 2 layers)} \\
LSTM layer norm                    & \multicolumn{3}{c}{True} \\
Fixed $\sigma$ (log $\sigma$ init) & \multicolumn{3}{c}{True ($\sigma = 1$)} \\
Optimizer                          & \multicolumn{3}{c}{Adam} \\
Learning rate (init)               & \multicolumn{3}{c}{$1 \times 10^{-4}$} \\
LR schedule                        & \multicolumn{3}{c}{Adaptive (KL-based)} \\
KL threshold                       & \multicolumn{3}{c}{0.008} \\
Mixed precision                    & \multicolumn{3}{c}{True} \\

\midrule
\multicolumn{4}{l}{\textbf{Environment / Other Training Settings}} \\
\midrule
Control decimation                 & \multicolumn{3}{c}{8} \\
Simulation timestep                & \multicolumn{3}{c}{$1/120$ s} \\
Control frequency                  & \multicolumn{3}{c}{$\sim$15 Hz} \\
Action space                       & \multicolumn{3}{c}{8 (6 pose + success + gripper)} \\
Save frequency                     & \multicolumn{3}{c}{20} \\
Episode length (s)                 & \multicolumn{3}{c}{20} \\
Episode length (steps)             & \multicolumn{3}{c}{300} \\
Number of parallel environments    &  \multicolumn{3}{c}{256} \\

\bottomrule
\end{tabular}
\vspace{1em}

\caption{Training hyperparameters shared across the three contact-rich pick-and-place
tasks (peg-insert, gear-mesh, nut-thread). Values spanning all columns are identical
for every task; the remaining rows list per-task settings.}
\label{tab:training_hyperparameters}
\end{table}

